CVE-driven Attack Technique Prediction with Semantic Information Extraction and a Domain-specific Language Model

This paper addresses a critical challenge in cybersecurity: the gap between vulnerability information represented by Common Vulnerabilities and Exposures (CVEs) and the resulting cyberattack actions. CVEs provide insights into vulnerabilities, but often lack details on potential threat actions (tactics, techniques, and procedures, or TTPs) within the ATT&CK framework. This gap hinders accurate CVE categorization and proactive countermeasure initiation. The paper introduces the TTPpredictor tool, which uses innovative techniques to analyze CVE descriptions and infer plausible TTP attacks resulting from CVE exploitation. TTPpredictor overcomes challenges posed by limited labeled data and semantic disparities between CVE and TTP descriptions. It initially extracts threat actions from unstructured cyber threat reports using Semantic Role Labeling (SRL) techniques. These actions, along with their contextual attributes, are correlated with MITRE's attack functionality classes. This automated correlation facilitates the creation of labeled data, essential for categorizing novel threat actions into threat functionality classes and TTPs. The paper presents an empirical assessment, demonstrating TTPpredictor's effectiveness with accuracy rates of approximately 98% and F1-scores ranging from 95% to 98% in precise CVE classification to ATT&CK techniques. TTPpredictor outperforms state-of-the-art language model tools like ChatGPT. Overall, this paper offers a robust solution for linking CVEs to potential attack techniques, enhancing cybersecurity practitioners' ability to proactively identify and mitigate threats.

==> Challenges.tex <==
\section{Challenges}
% there is no labeled data for training
% attack behavior requires context understanding
The most critical challenge of this work is the lack of labeled data. As of now, the only available data is 840 CVEs \footnote{\url{https://github.com/center-for-threat-informed-defense/attack_to_cve/blob/master/Att\&ckToCveMappings.csv}} mapped to a set of MITRE techniques and tactics by MITRE in which, labels do not precisely correspond to particular functionalities. Therefore, it is required to collect and annotate a standard dataset manually to train the predictive model. 

Data collection and annotation, on the other hand, are challenging problems since they require extensive text analysis to fully grasp the language structure of the target domain (CVEs) and to extract relevant text patterns for concise dataset generation.

The MITRE guideline-defined functionalities are not independent, and some of them may share similar characteristics. Thus, a single statement (e.g., a threat action) may have different implications in different contexts and correspond to multiple functionalities, which can lead to confusion and inconsistency during dataset generation and training. To distinguish similar texts, systematic data collection and a strategic training model design are required.
